ConceptMix: A Compositional Image Generation Benchmark with Controllable Difficulty

Compositionality is a critical capability in Text-to-Image (T2I) models, as it reflects their ability to understand and combine multiple concepts from text descriptions. Existing evaluations of compositional capability rely heavily on human-designed text prompts or fixed templates, limiting their diversity and complexity, and yielding low discriminative power. We propose ConceptMix, a scalable, controllable, and customizable benchmark which automatically evaluates compositional generation ability of T2I models. This is done in two stages. First, ConceptMix generates the text prompts: concretely, using categories of visual concepts (e.g., objects, colors, shapes, spatial relationships), it randomly samples an object and k-tuples of visual concepts, then uses GPT4-o to generate text prompts for image generation based on these sampled concepts. Second, ConceptMix evaluates the images generated in response to these prompts: concretely, it checks how many of the k concepts actually appeared in the image by generating one question per visual concept and using a strong VLM to answer them. Through administering ConceptMix to a diverse set of T2I models (proprietary as well as open ones) using increasing values of k, we show that our ConceptMix has higher discrimination power than earlier benchmarks. Specifically, ConceptMix reveals that the performance of several models, especially open models, drops dramatically with increased k. Importantly, it also provides insight into the lack of prompt diversity in widely-used training datasets. Additionally, we conduct extensive human studies to validate the design of ConceptMix and compare our automatic grading with human judgement. We hope it will guide future T2I model development.

==> sections/checklist.tex <==

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We provide the paper's contributions and scope and emphasizing the challenges of our benchmark in the abstract and introduction.}
  \item Did you describe the limitations of your work?
    \answerYes{We provide the limitation discussion in Sec.~\ref{subsec:limitation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We provide this discussion in Sec.~\ref{subsec:negative}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide the code, data and instruction needed in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We add the experiment details in the appendix Sec.~\ref{app:exp_detail}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the error bars in Tab.~\ref{tab:main}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide those details in Appendix Sec.~\ref{app:exp_detail}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite all of the works that we used in our work.}
  \item Did you mention the license of the assets?
    \answerYes{We mention that the LAION dataset we analyzed has MIT License}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Yes, we provide our dataset and coadebase in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All our data are generated and they are not from other people.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Our data are synthetic data and do not contain personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{We include them in Appendix~\ref{app:human_eval}.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \appendix



==> tables/categories.tex <==
\begin{table}[t!]
\vspace{-10mm}
\centering
\setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{Concept Categories in \evalname.} We collect eight diverse visual concept categories in \evalname to cover a wide range of visual concepts commonly used in compositional T2I generation. For each category, we provide definitions, concepts, and appearances in our text prompts.}
\resizebox{\linewidth}{!}{%
\small
\begin{tabular}{l|lll}
\toprule
\bfseries{Category} & \bfseries{Description} & \bfseries{Concepts} & \bfseries{Appearances in Text Prompts} \\
\midrule
\multirow{2}{*}{Objects} & generate  & \multirow{2}{*}{car, chair, sushi, etc. } &  A \textbf{woman} is holding a \textbf{ring} in her hand \\
& specific objects & &  A \textbf{table} with a \textbf{textbook} on it \\
\midrule
\multirow{2}{*}{Colors} & generate objects & \multirow{2}{*}{red, yellow, pink, etc.} & A single \textbf{blue} dog is present in the image. \\
& with specified colors. & & A \textbf{white} house stands alone. \\
\midrule
\multirow{2}{*}{Numbers} & generate specified & \multirow{2}{*}{two, three, four, etc.} & The image shows exactly \textbf{four} sheep standing on a grassy field. \\
& number of objects. & & \textbf{Three} laptops are placed side by side on a plain surface. \\
\midrule
\multirow{2}{*}{Shapes} & generate objects with & \multirow{2}{*}{circle, square, triangle, etc.} & An oak tree with a \textbf{heart-shaped} outline stands prominently in the scene. \\
& specified shapes. & &The image shows a \textbf{square-shaped} house. \\
\midrule
\multirow{2}{*}{Sizes} & generate objects with & \multirow{2}{*}{tiny, huge, etc.} & A \textbf{huge} cow is standing next to a sheep. \\
& specified sizes. & & A \textbf{tiny} textbook is placed on a chair. \\
\midrule
\multirow{2}{*}{Textures} & generate objects with & \multirow{2}{*}{metallic, glass, fluffy, etc.} &The image features a house with a \textbf{glass texture}. \\
& specified textures. & & A butterfly with a \textbf{fluffy texture} is perched on a surface. \\
\midrule
\multirow{2}{*}{Spatial} & generate objects with & \multirow{2}{*}{on top of, behind, inside, etc.} & The image shows a bench with an oak tree positioned \textbf{behind} it \\
& specified spatial relationships. & & A single bee is positioned on the \textbf{right} side of a flower. \\
\midrule
\multirow{2}{*}{Styles} & generate images with & \multirow{2}{*}{cartoon, sketch, watercolor, etc.} &  A \textbf{sketch} shows a single ring drawn with simple lines. \\
& specified artistic styles. & &The image shows a table drawn in an \textbf{ink} style. \\
\bottomrule
\end{tabular}%
}
\label{tab:categories}
\end{table}
